Personalized Showcases: Generating Multi-Modal Explanations for Recommendations

Existing explanation models generate only text for recommendations but still struggle to produce diverse contents. In this paper, to further enrich explanations, we propose a new task named personalized showcases, in which we provide both textual and visual information to explain our recommendations. Specifically, we first select a personalized image set that is the most relevant to a user's interest toward a recommended item. Then, natural language explanations are generated accordingly given our selected images. For this new task, we collect a large-scale dataset from Google Local (i.e.,~maps) and construct a high-quality subset for generating multi-modal explanations. We propose a personalized multi-modal framework which can generate diverse and visually-aligned explanations via contrastive learning. Experiments show that our framework benefits from different modalities as inputs, and is able to produce more diverse and expressive explanations compared to previous methods on a variety of evaluation metrics.

==> old_intro.tex <==
\section{Introduction}
% 1. interaction between user and business, items -> fine-grain
% 2. limitations of previous datasets, why we need a new dataset

% Comparing with two settings, POI or general item recommendation, explanation generation. 

\begin{figure}[t]
  \includegraphics[width=\linewidth]{images/intro.pdf}  
  \caption{Illustration of traditional business recommendation and our two proposed \data tasks, to provide personalized business (e.g.~restaurant) overviews that users are interested in. (1)~Personalized Showcase: to display a few images from reviews to 
  %satisfy 
  summarize
  users' different interests; (2)~Visually-Aware Explanation: to generate personalized natural language explanations about the given images. Compared with 
  %a 
  traditional business recommendation which only personalizes the
  %restaurant 
  item
  ranking, our tasks provide fine-grained 
  %personalized user experiences for 
  visual and textual explanations of
  business details.}
  \label{fig:intro}
  \vspace{-1em}
\end{figure}

%In daily life, 
Recommender systems 
%assist
help
users to 
%make decisions for interested \emph{business units} online or offline (e.g.,~
find relevant items, such as
which restaurant or 
%sight spot to visit). 
landmark to visit.
%Compared to single items, business units contain much richer information (e.g.,~dozens of dishes or decorations from a restaurant). 
%However, most current recommender systems only personalize the \emph{ranking} of business units according to users' historical behaviors (e.g.,~clicks, ratings) with non-personalized (thus less informative) business unit descriptions or reviews. 

To explore opportunities of \emph{finer-grained} personalization,
%for better user experiences, 
we propose a new multi-modal personalization pipeline for business units. 
That is, instead of only personalizing the business units ranking (\emph{coarse-grained}), our pipeline seeks to utilize users' and business units' historical (textual- and visual-) reviews to generates personalized multi-modal highlights of each business unit (\cref{fig:intro}).
%to meet various user interest. 
%As shown in~\cref{fig:intro}, when users browse restaurants and request more detailed information, our model offers personalized highlights for different users, saving them from overwhelming dishes descriptions and reviews.

To this end, we first construct a large-scale multi-modal dataset for business units personalization research. This new dataset, namely \data, is collected from \underline{G}oogleMaps\footnote{https://www.google.com/maps} R\underline{est}urant. 
\data\ includes 1,771,160 textual reviews with corresponding 4,435,565 user-generated photo urls. 
This dataset covers users' ratings, reviews from 1,010,511 users across 65,113 restaurants in 50 states in the US from $2012$ to $2021$. 
%The uniqueness of our dataset is that is a \emph{business-centric} \emph{multi-modal} review dataset.
Compared to existing multi-modal review datasets (e.g.,~Amazon Reviews~\cite{mcauley2015image}), our dataset focuses on reviews for businesses instead of single items, which remains new settings we can explore with finer-grained personalization; compared to existing \emph{bunisness-centric} review datasets (e.g.,~Yelp~\footnote{https://www.yelp.com/dataset}), ours contains rich textual- and visual- information generated from users. 
%So our dataset can not only contribute to conventional business recommendations or recommendation explanation generation tasks but also bring much richer information for broader applications, such as the proposed \emph{fine-grained} business personalization.

With 
%the new 
this
dataset, we then introduce two tasks for our \emph{fine-grained} business personalization pipeline: \textbf{(1)~Personalized Showcase}: to select several images from historical photos of this business that the user is most interested in (3-5 candidates on average)
%, may overload to users). 
Essentially, this can be formulated as an image recommendation task. \textbf{(2)~Visually-Aware Explanation Generation}: to generate natural language explanations given the displayed images and users' profiles (e.g.,~historical reviews). 
Explainable recommendation~\citep{Zhou2017LearningTG,lu2018like,li2020generate} can introduce richer information and improve user trust.
%the trust of users. 
%But c
Conventional single-modal explanation generators, as shown in~\citep{Ni2018PersonalizedRG}, tend to generate 
%some
general explanations (e.g.,~`food is good!'). In our multi-modal setting, with the grounding information from 
%specials
specific
images, explanation generation can be more concrete and informative (e.g.,~"steak is cooked well"). 

%Thus, compared to a conventional business recommendation or explanation generation, we propose a pipeline based on \data\ data consisting of the two tasks above, which will generate finer-grained personalized multi-modal information for users when they are interested in some businesses. 

Technically, for the first task, we propose a diversity-aware image personalized ranking model, to select relevant and diverse review images for different users. 
For the second task, we adopted a multi-modal GPT-2 model for explanation generation. We then show empirical studies of these two tasks separately and jointly. Overall, our contributions are three-fold:

\begin{itemize}
    \item We collect a new large-scale dataset for multi-modal, fine-grained personalization by crawling the web data from google maps restaurants.
    \item We introduce a novel pipeline for business-centric recommendation with two tasks, personalized showcase, and visual-aware explanation generation.
    \item We conduct comprehensive analysis and experiments to explore our dataset and validate the effectiveness of personalized features for two tasks.  
\end{itemize}


==> old_intro_1.tex <==
\section{Introduction}
% 1. interaction between user and business, items -> fine-grain
% 2. limitations of previous datasets, why we need a new dataset
% 3. Two tasks

\begin{figure}[t]
  \includegraphics[width=\linewidth]{images/intro.pdf}  
  \caption{Illustration of previous recommendation, text-only explanation and our personalized showcases. (1)~Previous recommendation only recommend items or businesses without rich information; (2)~Text-only Explanation models only use historical textual reviews from user and item sides to generate textual explanations. (3)~We propose a personalized showcases task to enrich the personalized explanations with multi-modal (visual and textual) information, which can largely improve the informativeness and diversity of generated explanations.}
  \label{fig:intro}
  \vspace{-1em}
\end{figure}

% 1. Previous works didn't have explanations. Textual explanations are not good enough. 
% 2. We propose the task (describing the task). Challenges in this task: Dataset and model. Previous datasets..., Hence, we collect a large-scale dataset from Google Locals.
% Different from the previous textual explanation generation, our showcases require both personalization and alignment of text and images.
% 3. To do this task, we propose a personalized cross-modal contrastive learning framework. In this framework,... .
% 4. From the experiments,...
% 5. Our contributions:

Recommender systems help users to find relevant items, such as which restaurant or landmark to visit. 
Previous works~\citep{He2017NeuralCF, He2017TranslationbasedR, Kang2018SelfAttentiveSR} focus on recommending items but doesn't provide rich information such as explanations about why items are recommended.
%recommended items. 
Explanations have the potential to increase the transparency and reliability of recommendations. To this end, previous works~\citep{Zhou2017LearningTG,Chen2019CoAttentiveML, Baheti2018GeneratingMI, Zang2017TowardsAG} 
considered generating textual explanations from users' historical reviews, tips~\citep{Li2017NeuralRR} or justifications~\citep{ni2019justifying}. However, these methods 
still struggle to provide diverse explanations because a large amount of general sentences (e.g.,~`food is good!') exist in user reviews and the text generation models lack grounding information for their generation process.

To explore opportunities for \emph{fine-grained} personalization and to further diversify and enrich explanations for recommendations,
we propose a new explanation generation task named \emph{personalized showcases}. 
In this new task, we explain recommendations via both textual and visual information. 
Compared to previous works that generate only text as explanations, our showcases present diverse explanations including images and visually-guided text. 
However, existing review datasets (e.g.,~Amazon~\citep{ni2019justifying} and Yelp\footnote{https://www.yelp.com/dataset}) 
are largely unsuitable for this
task~(we further discuss these datasets in~\Cref{sec:data-ana}). Thus, we first construct a large-scale multi-modal dataset, namely \data, which is collected from \underline{G}oogle Local\footnote{https://www.google.com/maps} R\underline{est}urants. 
\data\ includes 1,771,160 textual reviews with 4,435,565 corresponding user-generated photo urls and covers users' ratings, reviews from 1,010,511 users across 65,113 restaurants in 50 states in the US from $2012$ to $2021$. 
Then, to ensure the quality of generated explanations, we manually annotate a small dataset to find highly matched image-sentence pairs.
%that contains $9930$ image-text pairs whose images and text are highly matched 
Based on the annotations, we train a classifier with CLIP~\citep{Radford2021LearningTV} features to extract visually-aware explanations from the full dataset.
The photos and text explanations from users are used as the learning target for personalized showcases. 
Our task aims to provide a set of images that are relevant to a user's interest and generate textual explanations accordingly.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.99\linewidth]{images/example.pdf}
    \caption{Example of business and user reviews in \data. For a business (e.g.,~an Italian restaurant), \data contains historical reviews and images from different users.}
    \label{fig:reviews}
\end{figure*}

We design a pipeline for this new task~\footnote{We will release the code and datasets upon acceptance.}. First, we select several images from historical photos of the business that the user is most interested in. Then, we take the displayed images and users' profiles (e.g.,~historical reviews) as inputs and learn to generate textual explanations with a multi-modal decoder. %GPT-2~\citep{Radford2019LanguageMA}.

However, generate expressive, diverse and engaging texts that would arise users' interest remains a challenging problem. First, the input contains multiple images and historical reviews, which poses higher requirement for information extraction and fusion across modalities.  
Second, a typical encoder-decoder model with cross-entropy loss and teacher forcing can easily lead to generating repetitive and dull sentences that occurs frequently in the training corpus (e.g., ``food is great'')~\citep{holtzman2019curious}.

To tackle these issues, we propose a \textbf{P}ersonalized \textbf{C}ross-Modal \textbf{C}ontrastive \textbf{L}earning ($PC^2L$) framework by contrasting input modalities with output sequences. 
Contrastive learning has drawn attention as a self-supervised representation learning approach. 
However, simply training with negative samples in a mini-batch is suboptimal~\citep{chen2020simple,lee2020contrastive} for many tasks, as the randomly selected embeddings could have been well-discriminated in the latent space. 
Hence, we first design a cross-modal contrastive loss to enforce the alignment between images and output explanations, by constructing hard negative samples with randomly replaced entities in the output.
Motivated by the observation that users with similar historical reviews share similar interest, we then designed a personalized contrastive loss to reweight the negative samples based on their history similarities.
Experimental results on both automatic and human evaluation show that our model is able to generate more expressive and diverse explanations comparing to a variety of baselines.

% We conduct experiments on \data and compare the single-modal (i.e.~text only) explanation generation models to our multi-model (i.e.,~text and image) showcase pipeline. We find that the textual explanations from our showcases are more diverse ($22\%$ on Distinct-1 and $45\%$ on Distinct-2) than explanations generated from single-modal methods. 
% In addition to the diversity for text generation, we argue that the ability to align images and explanations should also be considered. 
% Hence, we further design a new CLIP-based metric to measure the visual alignment. 
% We further conduct human evaluation and case studies to demonstrate the textual explanations from our showcases are more informative to users.

Overall, our contributions are concluded 
%into three folds:
as follows:
\begin{itemize}
    \item To have fine-grained personalization and generate more informative explanations for recommendations, we propose a new task: \emph{personalized showcases} which can provide both textual and visual explanations for recommendations.
    
    \item For this new task, we collect a large-scale multi-modal dataset from \emph{Google Local} (i.e.,~maps). To ensure 
    alignment between images and text, we annotate a small dataset and train a classifier to propagate labels on \data, and construct a subset for generating textual explanations.
    
    \item We propose a novel contrastive learning framework for personalized showcases. Comprehensive experiments on both automatic and human evaluation indicate that textual explanations from our showcases are more expressive and diverse than exsiting explanation generation methods. 
\end{itemize}



